Encryption without Centralization: Distributing DNS Queries Across Recursive Resolvers

Emerging protocols such as DNS-over-HTTPS (DoH) and DNS-over-TLS (DoT) improve the privacy of DNS queries and responses. While this trend towards encryption is positive, deployment of these protocols has in some cases resulted in further centralization of the DNS, which introduces new challenges. In particular, centralization has consequences for performance, privacy, and availability; a potentially greater concern is that it has become more difficult to control the choice of DNS recursive resolver, particularly for IoT devices. Ultimately, the best strategy for selecting among one or more recursive resolvers may ultimately depend on circumstance, user, and even device. Accordingly, the DNS architecture must permit flexibility in allowing users, devices, and applications to specify these strategies. Towards this goal of increased de-centralization and improved flexibility, this paper presents the design and implementation of a refactored DNS resolver architecture that allows for de-centralized name resolution, preserving the benefits of encrypted DNS while satisfying other desirable properties, including performance and privacy.

==> sections/conclusion.tex <==
\section{Conclusion}
TODO; this is just a placeholder


==> sections/principles.tex <==
\section{Designing for Tussle}
\AH{Although this version of the paper is likely going to be focused on addressing centralization, rather than the various tussle spaces that exist in the DNS, Clark's principles (or a subset of them) may still be useful for us. We may be able to apply them to how centralization as a particular tussle space could be addressed. However, right now this section kind of awkwardly appears. We probably need some new section title and introductory text to ease the reader into why we're talking about Clark's ideas in the context of DNS centralization. One way of doing so is adding a paragraph that says the following: 1) what is a tussle, 2) how is DNS centralization a tussle, and 3) how are Clark's principles relevant}

\AH{Implications for the DNS -> Implications for addressing DNS centralization}
In this section, we outline Clark et al.'s principles for designing for
tussle~\cite{clark2002tussle} and explain their implications for the DNS.

\subsection{Design for Choice}
\paragraph{Definition.}

To address tussles over Internet protocols, Clark et al. argue that protocols
should be designed such that users can choose who they communicate and
exchange data with:  

\begin{quote} Network protocols are designed so that different parties on the
    network can communicate with each other, consumers can make use of the
    resources of providers, and providers can interconnect with each other to
    provide service.  It is important that protocols be designed in such a way
    that all the parties to an interaction have the ability to express
    preference about which other parties they interact with.  Protocols must
    permit all the parties to express choice~\cite{clark2002tussle}.
\end{quote}

\AH{Implications for DNS -> Implications for DNS Centralization}
\AH{Re-word text about "addressing DNS tussles"}
\paragraph{Implications for DNS.} When addressing DNS tussles (\eg, users
not placing trust in a particular resolver), we not only interpret ``design for
choice'' to mean that users should always be able to decide how DNS resolution 
is performed, but also that DNS configuration options should 
be presented in ways that are meaningful to users.
Users should then be able to apply these configurations across any
application on a device.
Applications (or devices acting in the interests of their designers) should not 
be able to choose where DNS resolution is performed that violate users' wishes 
or in ways that users cannot override.

Many scenarios in today's Internet are not designed for choice. For example,
Google Chromecast has reportedly used Google's public DNS resolver by
default, and has lost function if network operators force another resolver 
to be used~\cite{nest_dns}. Users can technically set up a resolver on the local 
network to respond to queries destined for Google's resolver, but this requires 
significant expertise and is not a feasible choice for most users. The lack of choice in DNS resolution has significant implications
for privacy and reliability. Users may not trust Google (or other resolvers)
with their DNS queries, raising concerns about how users' data is handled
against their wishes.  Furthermore, if Google's own DNS resolver fails and
clients have no feasible way of choosing other resolvers, then Google's devices 
that are hard-coded to use their resolver may lose function.

Users may be unaware of the DNS and the implications of
choosing between DNS resolvers in the first place.  However, users that desire
to make these choices should at least be able to.  This may be
difficult to achieve on embedded devices or on the ``Internet-of-Things'' (IoT),
but without visibility of what choices are made and the ability
for users to make choices for themselves, the tussle between users and
resolvers over trust will continue. Moreover, these choices should be presented 
in ways that are meaningful to users. For example, if users are presented 
with a dialog box by an application or stub resolver asking if they wish to 
enable encrypted DNS, the dialog box should attempt to inform users what the 
privacy implications are for enabling encrypted DNS with a particular resolver.

% We also argue that designing for choice in the DNS implies that recursive
% resolvers should be able to express information about themselves to clients.
% This information would enable DNS clients to make meaningful choices among
% numerous possible recursive resolvers, including input from users.  For
% example, a recent IETF draft proposes a mechanism that enables the local
% network to express privacy policies for a local resolver over DHCP in a
% machine-readable format.  This data could enable operating systems and
% applications that perform DNS resolution to make decisions about whether a
% local resolver should be used over other known resolvers.  Although this
% draft has not been standardized, we believe it is a promising idea that
% might enable clients to make more meaningful decisions about DNS resolution.
% \AH{Cite the IETF draft later}


\subsection{Don't Assume the Answer} \paragraph{Definition.} Clark et al. also
argue that when it comes to Internet architectures and protocols, ``there is no
such thing as value-neutral design'': 

\begin{quote} What choices designers include or exclude, what interfaces are
    defined or not, what protocols are open or proprietary, can have a
    profound influence on the shape of the Internet, the motivations of the
    players, and the potential for distortion of the architecture. Don't
    assume that you design the answer. You are designing a playing field, not
    the outcome~\cite{clark2002tussle}.  \end{quote}

\begin{figure}[t!]
    \centering
    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \raisebox{2mm}{
            \includegraphics[width=\textwidth]{figures/ff-popup-1}}
        \label{fig:ff-popup-1}
        \caption{February 2020}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/ff-popup-2}
        \label{fig:ff-popup-2}
        \caption{September 2020}
    \end{subfigure}
    \caption{Firefox pop-up menus for opting out of encrypted DNS have changed
    over time. Initially, Cloudflare was explicitly mentioned. Over time, the
    consequences of this opt-out choice became more opaque to users}
    \label{fig:ff-popup}
\end{figure}

\AH{Implications for DNS -> Implications for DNS Centralization}
\paragraph{Implications for DNS.} DNS clients can select resolvers in a
variety of ways, rather than designing a ``playing field'' As previously
discussed, various applications and devices have made default choices for
recursive resolvers that have been met with criticism.  When Google configured
its Chromecast devices to use their own recursive resolver, rather than the
resolvers advertised by local networks, they assumed the answer, designing an
outcome that not only restricted user choice, but also led to increased
concerns over privacy and reliability.  Similarly, when Mozilla launched its
trusted recursive resolver program for DoH in the United States with
Cloudflare as the default recursive resolver, users expressed concern over DNS
centralization at an entity separate from their default DNS providers.  Users
were presented with a choice via a one-time, obscure pop-up menu, to opt out
of using DoH (and Cloudflare's resolver) by default, DNS (and in turn, DoH),
as shown in Figure~\ref{fig:ff-popup}; over the course of 2020 this option
became more obscure, and in Firefox 85.0, the option was enabled by default
with no opt-out. 
Disabling or changing these default settings is possible, but the options are
buried multiple levels deep in configuration menus that users likely aren't
even aware of. Figure~\ref{fig:dropdown} shows the configuration menus in
Firefox and Brave, as well as the default configurations for each.

\begin{figure}[t!]
    \centering
    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \raisebox{2mm}{
            \includegraphics[width=\textwidth]{figures/ff-dropdown}}
        \label{fig:ff-dropdown}
        \caption{Firefox}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.48\linewidth}
        \centering
        \includegraphics[width=\textwidth]{figures/brave-dropdown}
        \label{fig:brave-dropdown}
        \caption{Brave}
    \end{subfigure}
    \caption{Different browsers have different default settings for DNS
    resolution; most users are likely unaware of these options and wouldn't
    even understand them even if they could find them at all.}
    \label{fig:dropdown}
\end{figure}

\AH{We don't implement behavior for choosing different resolvers based on geographic location, 
so this text may be too philosophical for ANRW.}
DNS clients can instead design for a playing field among resolvers instead of
a particular outcome that may surprise users. If applications ultimately
decide to choose resolvers that were not advertised by the local network, in
addition to offering choice to users, in some cases it may also be appropriate
to assign different default resolvers to different populations of users by
default.  For example, Mozilla's deployment of the trusted recursive resolver
program with Cloudflare as the default provider for Europe was problematic,
since Cloudflare is a United States-based company, and European users can have
different expectations---and regulations---governing data protection
practices.  Although Mozilla has yet to roll out its trusted recursive
resolver program to European users, there is nonetheless significant concern
that a single resolver (or small set of resolvers) that was designed for
United States users will be configured for European users.
\AH{Not sure if Mozilla is planning to roll out Cloudflare DoH to Europe.}
Other regions may also have unforeseen circumstances where assuming a particular answer may
defy norms or catch users by surprise.

\AH{We don't implement a configuration option that enables clients to prefer local DoH resolvers 
over public resolvers on particular networks, so we may want to remove that text for ANRW. However, we could 
keep the text about splitting queries across multiple resolvers.}
Applications and devices should not assume the answer, and they should
especially not assume that one answer suffices for all users. They should enable
users to express preferences about resolver selection when multiple choices
are available.  For example, when a local resolver supports DoH and the
application/device also knows of multiple public resolvers that also support
DoH, clients may want the local resolver to take precedence.  Other clients
may want public resolvers to take precedence, only using the local resolver
when the configured public resolvers are unavailable.  Some clients
may even wish to split their queries across multiple recursive resolvers,
preventing any single resolver from having access to all of their queries.
In short, clients should be able to express preferences about how to select
between multiple recursive resolvers---making fine-tuned decisions about how
their queries are resolved---rather than only sending queries to a single
resolver by default.

\subsection{Modularize Along Tussle Boundaries} \paragraph{Definition.} Finally,
Clark et al. argue for breaking the Internet architecture into modular 
components when possible, such that tussles over one part of the architecture 
do not spill over into other parts:

\begin{quote}
    Functions that are within a tussle space should be logically separated from 
    functions outside of that space, even if there is no compelling technical 
    reason to do so. Doing this allows a tussle to be played out with 
    minimal distortion of other aspects of the system’s function
    ~\cite{clark2002tussle}.
\end{quote}

\AH{Implications for DNS -> Implications for DNS Centralization}
\paragraph{Implications for DNS.} 
Traditionally, operating systems have performed DNS resolution on behalf of 
applications running on a device.
Today, applications themselves can make their own decisions about which DNS 
transports and recursive resolvers should be used, independent of what the 
operating system learns from the network or configures on its own.
Entire devices have also reportedly ignored the DNS configurations 
learned from the network~\cite{nest_dns}. Such behavior prevents all 
stakeholders the potential to access DNS data.
Users that wish to change how DNS resolution is performed on their devices 
may now need to make changes in multiple locations \eg, in both the web 
browser and the operating system's stub resolver.
\AH{Say something about how having to make changes in multiple places makes it harder 
for clients to decide where their DNS queries go}

\AH{Add some text about running a stub resolver on a router to make decisions for the whole network. 
We have to be careful in our wording, though, because making decisions for a whole network could be 
interpreted as contributing to DNS centralization, e.g. if we choose Google's resolver for a large 
population of users.}
If each application on a device handles recursive resolver selection in a different
way, then DNS tussles over privacy, trust, centralization, and reliability
will continue. 
%\footnote{Currently,
%there is no standardized mechanism to learn that a local resolver supports
%encrypted DNS. Nonetheless, when such functionality becomes available, 
%applications should rely on the operating system to perform
%encrypted DNS resolution and resolver selection on their behalf.} 
Applications may not trust local resolvers and may
wish to always use encrypted DNS, but users wish to override the decisions
made by the applications, then they will need to make changes in multiple
locations instead of one and will continue to have little visibility into
the decisions that each application makes.

\if 0
Operating systems have traditionally performed the
role of DNS resolution, so what we are arguing for is not necessarily a new
concept.  However, with various applications making different decisions about
how to perform encrypted DNS resolution, users no longer have a consistent
picture of which parties have access to their DNS data.  In a sense, we are
arguing for a \emph{return to form} so that stakeholders--users, ISPs and
public resolvers--can exert their influence in a single, well-defined
location.
\fi


==> sections/related.tex <==
\section{Related Work}



==> sections/stakeholders.tex <==
\section{Tussle Spaces in (Encrypted) DNS}

Encrypted DNS has provoked tussles between various participants in the Internet
ecosystem: users, who want good performance (and privacy); Internet service
providers (ISPs), who often leverage DNS as a control plane for security and
performance reasons, and may wish to infer customer behavior; content delivery
networks, who use user DNS information to localize users to nearby content
replicas; and public resolvers, who may use DNS queries to learn about user
behavior. In this section, we explore the tussles concerning (encrypted) DNS in
more detail, explain how the current architecture fails to resolve (and in some
cases, exacerbates) them, and suggest various approaches for designing DNS
architecture to account for these tussles.

\subsection{Users vs. Public Resolvers \& ISPs}
\paragraph{Who Are The Stakeholders?}
The operators of many large commercial public resolvers---notably Google and
Cloudflare---have an incentive to observe (and resolve) users' DNS queries, due
to benefits garnered for content delivery, advertising, or both. Likewise, ISPs
have an interest in observing and resolving DNS queries because they use the
information for security purposes, as well as to implement various products like
parental controls. Users not only desire a DNS resolver that performs well, but
also one that doesn't track them or manipulates responses. The rest of this
section explores this tussle.

\paragraph{What Is The Tussle?}
Public resolvers have seen increased usage in recent years, spurred on by their
early adoption of encrypted DNS. Some users may not trust public resolvers with
their DNS data, however. When Mozilla announced that Cloudflare would be the
initial default recursive resolver for their DoH rollout to Firefox desktop
users in the United States, users expressed concern over Cloudflare's potential
motivations for participating in the program~\cite{hubert2019centralised}. Some
argued that the program would centralize DNS data at Cloudflare, raising
concerns about robustness, competition, and privacy. On the other hand,
researchers have found that Google's public resolver already sees a
comparatively large portion of DNS queries over any other DNS
resolver~\cite{moura2020clouding}. Thus, some may argue that the DNS is
\emph{already} centralized into a handful of resolvers. At the same time, as
ISPs begin to deploy encrypted DNS, other users may not want their ISP to see
all of their DNS queries, either.

\paragraph{Why Hasn't The Tussle Resolved?}
Most stub resolvers and applications that support encrypted DNS send all of a
users' queries to a single recursive resolver that is configured on the
operating system or by an application that embeds a stub resolver. Some users
have expressed concern over coupling their queries with a single resolver
because it may enable an operator to track their browsing histories over time.
Although most users tend to not know about the DNS and its implications, we
argue that for centralization to be truly addressed--whether at an ISP or a
public recursive resolver--users need some way of meaningfully expressing
preferences regarding privacy and availability. We recognize that many resolvers
send queries to additional resolvers as a fallback mechanism, but this is not
the proactive distribution of queries that we envision. Furthermore, this
behavior is not for trust or privacy purposes, but rather for reliability.

\subsection{Public Resolvers vs. Each Other}
\paragraph{Who Are The Stakeholders?}
Many organizations operate publicly available recursive resolvers, which users
can use to perform DNS resolution on their behalf. Although there are hundreds
of public DoH recursive resolvers, only a few TRRs---notably, Google,
Cloudflare, and Quad9---are optimized for large-scale deployment. In many cases,
these organizations have an incentive to access more DNS queries and serve more
users for various commercial purposes. First, they may use the brand recognition
of these resolvers to lead customers to other products that they offer. Second,
they may analyze the contents of DNS queries to determine which websites users
are visiting. This data could then be used to track users, to deliver targeted
advertising, or sold to third parties. Third, certain public resolvers are
hosted by content delivery networks (CDNs), who may use DNS queries to localize
users and direct them to nearby content caches.

\paragraph{What Is The Tussle?}
Commercial organizations that operate public recursive resolver compete with one
another and hence compete for users' DNS queries. Cloudflare and Google both
operate content delivery networks; Comcast, who recently launched a TRR service,
also delivers its own content (Comcast is owned by NBC Universal). To improve
the performance of the delivery of content on their own CDNs, Cloudflare and
Google may use DNS data to direct users to their local caches. ISPs who operate
recursive resolvers may offer additional services, such as malware
protection or parental controls, that depend on seeing DNS traffic. Large
operators of public resolvers are thus tussling over which party gets to see
users' DNS queries and enjoy the benefits of improved performance to their own
services.

% It should be noted that Cloudflare and Google already own a significant market share over recursive resolvers.
% APNIC runs continuous measurements through scripts embedded in online advertisements to estimate the popularity of various recursive resolvers.
% For December 2020, they estimate that Google's public recursive resolver is responsible for X\% of queries seen by an authoritative server that APNIC operates~\cite{apnic-centralization}.
% Other researchers ran measurements in 2020 that estimate that Cloudflare and Google's recursive resolvers are responsible for X\% of queries issued to the \texttt{.nl} and \texttt{.nz} zones~\cite{imc2020centralization}.
% Thus, the competition between Cloudflare and Google has already resulted in significant centralization of DNS data.
% \AH{Fill in numbers and citations later. Also, we may want move this paragraph to the introduction. Depends on what direction we take it.}

\paragraph{Why Hasn't The Tussle Resolved?}
Despite the fact that there are hundreds of DoH resolvers
deployed~\cite{dnscrypt_resolvers}, only a few DoH resolvers are currently
available as options in Firefox. Mozilla's trusted recursive resolver (TRR)
program requires DoH resolvers to agree to specific requirements, to be listed
in an (obscure) drop-down menu in the browser configuration. Approved TRRs must
not retain DNS logs for more than 24 hours, and these logs cannot be sold or
shared with other parties~\cite{trr_program_blog}. Although this program may be
ultimately be beneficial to users' privacy, it affects competition between
resolvers and effectively makes the browser vendor the gatekeeper for which
organizations can participate in the DNS tussle space.

This arrangement favors some incumbents, while balkanizing the tussle space
along various market segments. Notably absent from Mozilla's TRR program is
Google's public DoH resolver (one can intuit from this fact that Google may be
logging users' DNS queries). Thus, if users wish to use Google's DoH resolver in
Firefox, they must manually configure it, even if Google is already configured
as their unencrypted DNS resolver at the operating system level. No matter, of
course: Google operates Chrome, the dominant Web browser, and has less of a need
to join Mozilla's program in the first place. Such a dynamic further cements the
centralization of companies that control large portions of the market. As of May
2020, Google Chrome assigns users to a DoH resolver that is consistent with the
user's preferences and settings~\cite{chrome_doh_upgrade_blog}. If Chrome finds
that the DNS resolver configured on a user's operating system is included in a
pre-defined table of DoH resolvers, then Chrome will assign that user to the
corresponding DoH resolver. Such behavior can change at any time, of
course---often with obscure or no notification to the user---as it did with
Mozilla's rollout of a default DoH configuration last year.


\subsection{Public Recursive Resolvers vs. ISPs}
\paragraph{Who Are The Stakeholders?}
Despite the increasing popularity of public resolvers, users primarily use the
resolvers that are advertised by their ISPs. ISPs may operate these resolvers
for various reasons. For example, they might use these resolvers to provide
parental controls for their customers or automatically block DNS-based malware.
They may also operate resolvers to improve network performance for their
customers by running a local DNS cache. Finally, they may use this data for
commercial purposes, for example to re-direct customers to landing pages with
advertisements when they mistype a URL~\cite{comcast_domain_helper}.

\paragraph{What Is The Tussle?}
Given the historical role of ISPs in providing DNS resolution, ISPs are
resistant to the increasing popularity of public resolvers. The debate between
ISPs and public resolvers over who should perform DNS resolution has recently
played out in web browsers. When Mozilla announced that they were enabling DoH
by default in 2020, Cloudflare and NextDNS were the default recursive
resolvers~\cite{doh_rollout_faq_mozilla} Some have argued that by choosing a few
resolvers as the default providers, Mozilla is enabling DNS data to be
increasingly centralized into a handful of organizations, rather than the
historical multitude of ISPs. Further, as of January 2021, Google Chrome only
performs auto-upgrade for a few major ISP DoH resolvers, \eg, Comcast and
Spectrum~\cite{chrome_doh_upgrade_providers}. ISPs contend that current
deployment models of DoH favor large public resolvers over ISPs. In 2020,
Comcast announced a collaboration with Mozilla to deploy their recursive
resolver to Firefox users that use Comcast's
networks~\cite{comcast_trr_announcement}. Comcast would become a member of
Mozilla's trusted recursive resolver program, agreeing to audits of their DNS
data and various privacy requirements; however, as of January 2021 (Firefox
85.0), Comcast is still not listed as a TRR option. 

\paragraph{Why Hasn't The Tussle Resolved?}
ISPs sometimes argue that Mozilla and Google should not have offered DoH
resolution before a local DoH resolver discovery mechanism was standardized. As
of January 2021, several mechanisms have been proposed within the Adaptive DNS
Discovery IETF working group to support local DoH resolver discovery, but they
have not yet been standardized~\cite{ietf_add_documents}. As a result,
customization remains cumbersome and obscure: users can only use an ISP's DoH
resolver is if they know the information for the resolver in advance and
configure the resolver manually. It remains unclear whether users that use ISPs
that are a part of Mozilla's trusted recursive resolver program will exclusively
be assigned to use the ISP-provided resolvers, or share queries across third
party public recursive resolvers as well. It is also unclear which ISP resolver
Firefox will use when users switch between networks whose DNS resolvers are all
members of the trusted recursive resolver program.

